Self-supervised Training Sample Difficulty Balancing for Local Descriptor Learning

In the case of an imbalance between positive and negative samples, hard negative mining strategies have been shown to help models learn more subtle differences between positive and negative samples, thus improving recognition performance. However, if too strict mining strategies are promoted in the dataset, there may be a risk of introducing false negative samples. Meanwhile, the implementation of the mining strategy disrupts the difficulty distribution of samples in the real dataset, which may cause the model to over-fit these difficult samples. Therefore, in this paper, we investigate how to trade off the difficulty of the mined samples in order to obtain and exploit high-quality negative samples, and try to solve the problem in terms of both the loss function and the training strategy. The proposed balance loss provides an effective discriminant for the quality of negative samples by combining a self-supervised approach to the loss function, and uses a dynamic gradient modulation strategy to achieve finer gradient adjustment for samples of different difficulties. The proposed annealing training strategy then constrains the difficulty of the samples drawn from negative sample mining to provide data sources with different difficulty distributions for the loss function, and uses samples of decreasing difficulty to train the model. Extensive experiments show that our new descriptors outperform previous state-of-the-art descriptors for patch validation, matching, and retrieval tasks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> figure tex/Table1.tex <==



\begin{table}[hp] \scriptsize%此处将表格字体设置为tiny，也可以设置为其它大小
                        %%参数： h:放在此处 t:放在顶端 b:放在底端 p:在本页
		\centering
		\renewcommand\arraystretch{1.2}
		%\setlength{\abovecaptionskip}{0.cm}
		%\setlength{\belowcaptionskip}{-0.cm}
		% 显示位置为中间	
		\label{tabl:Abl}  % 用于索引表格的标签
		%\caption{	}  % 表格标题
		\textbf{Table 1} \\  %%表的标题
		
		\begin{tabular}{>{\centering}p{80pt}|c|c} %第一列设置宽度为45pt 全为左对齐 没有分割线
			%\setlength{\tabcolsep}{20mm}
			%\hline  % 表格的横线
			%\toprule % 顶部线
			Modification & Choice & MAP(\%) \\%[3pt]只改一行    %%表格第一行标题 % 表格中的内容，用&分开，\\表示下一行
			\hline  % 表格的横线
			
			\multirow{2}{*}{\textbf{Loss function}} & HardNet loss & 55.67\\
			\multirow{2}{*}{} & Balance loss & 56.53\\
			\hline
			
			\multirow{2}{*}{\textbf{{\makecell[c]{Teacher net\\outliers handling}}}} & HardNet loss+TNet &  56.08\\
			\multirow{2}{*}{} & Balance loss+TNet & 56.83\\
			\hline
			
			\multirow{3}{*}{\textbf{{\makecell[c]{Annealing\\training}}}} & AN+HardNet loss +TNet & 56.25\\
			\multirow{3}{*}{} & AN+Balance loss & 57.01\\
			\multirow{3}{*}{} & AN+Balance loss+TNet  & 57.35\\
			\hline
% 			\multirow{2}{*}{\textbf{{\makecell[c]{Descriptor\\type}}}} & {\multirow{2}*{\makecell[c]{Hard+FRN\\SOSNet+FRN}}} &\\
% 			\multirow{2}{*}{} & {\multirow{2}*{}}& \\
% 			\hline
			%\bottomrule % 底部线
			%\hline  % 表格的横线
		\end{tabular}
	\caption{在HPatch匹配任务上的消融实验。数据集为full split}  % 表格标题
	\end{table}

==> figure tex/not used/Fig_bs_thr_inAT.tex <==
% \pgfplotsset{width=8cm,height=6cm,compat=1.5}% <-- moves axis labels near ticklabels (respects tick label widths)


    \begin{tikzpicture}
			\begin{axis}[
				title={},
				xlabel={$stepwise_{bs}$},
				ylabel={MAP($\%$)},
				xmin=-0.01, xmax=0.17,
				ymin=55.4, ymax=57.4,
				xtick={ 0, 0.05, 0.10, 0.15},
                xticklabels={$128$,$192$,$256$,$0.15$},
				ytick={55.5, 56.0, 56.5, 57.0},
				% legend pos=north,
                    legend style={at={(0.55,0.98)},
	            anchor=north, legend columns=2},
				xmajorgrids=true,
				ymajorgrids=true,
				grid style=dashed,
				]
			 % \addplot
% 				coordinates {
% % 					(0,51.9)
% % 					(1,53.5)
% % 					(2,54.1)
% % 					(3,53)
% % 					(4,52.5)
% 				};
        	\addplot
				coordinates {
					(0, 56.2895)
					(0.05, 56.4555)
					(0.1, 56.0203)
					(0.15, 56.4031)
				};
				\addplot        %thr=-0.5
				coordinates {
 					(0,55.8)
 					(0.05,55.86215)
 					(0.1,56.2727)
					(0.15,56.5319)
				};

				\addplot        % thr=-0.65
				coordinates {
					(0, 56.5772)
					(0.05,56.5987)
					(0.1,56.3412)
					(0.15,56.5227)
				};
                \addplot
				coordinates {
					(0, 56.401)
					(0.05, 56.4171)
					(0.1, 56.0203)
					(0.15, 55.7882)
				};
				\legend{thr=-0.35, thr=-0.5,  thr=-0.65, thr=-0.80}
			\end{axis}
		\end{tikzpicture}
